TinyQMIX: Distributed Access Control for mMTC via Multi-agent Reinforcement Learning

Distributed access control is a crucial component for massive machine type communication (mMTC). In this communication scenario, centralized resource allocation is not scalable because resource configurations have to be sent frequently from the base station to a massive number of devices. We investigate distributed reinforcement learning for resource selection without relying on centralized control. Another important feature of mMTC is the sporadic and dynamic change of traffic. Existing studies on distributed access control assume that traffic load is static or they are able to gradually adapt to the dynamic traffic. We minimize the adaptation period by training TinyQMIX, which is a lightweight multi-agent deep reinforcement learning model, to learn a distributed wireless resource selection policy under various traffic patterns before deployment. Therefore, the trained agents are able to quickly adapt to dynamic traffic and provide low access delay. Numerical results are presented to support our claims.

==> section/_/decpomdp.tex <==
\subsection{Problem formulation for cooperative multi-agent tasks}

A \emph{cooperative multi-agent learning problem} can be formulate as a \gls{decpomdp} \cite{oliehoek2016concise}, which is defined as a tuple $G = \langle n, S, U, P, r, Z, O, \gamma \rangle$.
The system consists of $n$ agents.
$s \in S$ is the true state of the environment.
In every timeslot, each agent $i \in \{1, \ldots, n\}$ chooses an action $u^i \in U$.
The actions of all agents constitute the joint action $\vb{u} = (u^1, \ldots, u^n) \in U^n \equiv \vb{U}$.
If the joint action is $\vb{u}$ under the state $s$, the next state of the system $s^{'}$ can be obtained according to the state transition function $P(s^{'}|s, \vb{u}): S \times \vb{U} \rightarrow \vb{S}$.
Let $r(s, \vb{u}): S \times \vb{U} \rightarrow \mathbb{R}$ be the reward function and $\gamma \in [0, 1)$ is the discount factor.

\emph{Partially observable} means that each of $n$ agents cannot obtain the true state $s$, but they can extract their individual observation $z \in Z$ based on the observation function $O(s, a): S \times A \rightarrow Z$.
Each $i^{t}$ agent has an action-observation trajectory $\uptau^i \in \mathcal{T} \equiv (Z \times U)^{*}$, on which it conditions a stochastic policy $\pi^i(u^i|\uptau^i): \mathcal{T} \times U \rightarrow[0, 1]$.
The joint policy $\pi$ has a joint action-value function $Q^{\pi}(s_t, \vb{u}_t) = \mathbb{E}_{s_{t+1:\infty}, \vb{u}_{t+1:\infty}} [R_t|s_t, \vb{u}_t]$, where $R_t=\sum_{t^{'}=0}^{\infty} \gamma^{t^{'}} r_{t+t'}$ is the long term discounted return.
The goal of the whole multi-agent system is to maximize the long term discounted return.


==> section/_/dqn.tex <==
\subsection{Deep Q-Networks}

\gls{dqn} captures the action-value function $Q(s, \vb{u})$ using a \gls{dnn} $Q(s, \vb{u}; \theta)$ \cite{mnih2015human}.
Particularly, input to the \gls{dnn} is the state $s$, and each discrete output of the \gls{dnn} corresponds to each joint action's expected discounted return.
While the \gls{dnn} is training, it retains a replay memory $\mathcal{M}$ contains many transitions $\langle s, \vb{u}, r, s^{'}\rangle$.
$\theta$ is updated by minimizing the expected squared temporal different error given the data in the replay memory:
\begin{equation}
    \mathcal{L}(\theta) = E_{\langle s, \vb{u}, r, s^{'} \rangle \sim \mathcal{M}} \bigg[ \bigg(Q^{target}- Q(s, \vb{u}; \theta) \bigg)^2 \bigg]
\end{equation}
where the target action-value is
\begin{equation}
    Q^{target} = r + \gamma \max_{\vb{u}^{'}} Q(s^{'}, \vb{u}^{'}; \theta^{-})
\end{equation}
and $\theta^{-}$ is the parameter of a target network, which is periodically copied from $\theta$ to make the target action-value become more stable.



==> section/_/index.tex <==
% \section{Background}

% This section reviews the \gls{decpomdp} formulation for cooperative multi agent learning and techniques to solve this decision process.
% They are the backbone to our proposed decentralized resource allocation \gls{mtc} system.

% \input{section/background/decpomdp}
% \input{section/background/dqn}
% \input{section/background/qmix}


==> section/_/qmix.tex <==
\subsection{QMIX}
\label{sec:background:qmix}

\gls{qmix} \cite{rashid2018qmix} is a recently proposed multi-agent learning method for solving \gls{decpomdp}.
Let $Q_{tot}(\boldsymbol{\uptau}, \vb{u})$ be the joint action-value function, where $\boldsymbol{\uptau} \in \mathcal{T}^{n} \equiv \boldsymbol{\mathcal{T}}$ is the joint action and local observation history (joint of $u^i$ and $z^i$).
Each $i^{th}$ agent has its own utility function $Q_i(\uptau^i, u^i; \theta^i)$, which evaluate its own action on local observations only.
This enables each agent to execute decentrally without communicating to a centralized planner.
However, the whole multi-agent system could descent into anarchy if there is no constraint imposing to the individual utility functions $Q_i$.
Therefore, \gls{qmix} ensures that all agents's utility function is consistent with the centralize joint action-value function, such that:
\begin{equation}
    \underset{u}{\text{argmax }} Q_{tot}(\boldsymbol{\uptau}, \vb{u}) = 
    \begin{pmatrix}
        \underset{u^1}{\text{argmax }} Q_1(\uptau^1, u^1)\\
        \vdots\\
        \underset{u^n}{\text{argmax }} Q_n(\uptau^1, u^1)\\
    \end{pmatrix}
    \label{eq:qmix:constraint}
\end{equation}
Inparticular, the constraint is realize using a mixing networks, which is a fully connected \gls{dnn} with the inputs is a vector combining all individual utility functions $Q_i(\uptau^i, u^i; \theta^i)$ to produce the output $Q_{tot}$ such that:
\begin{equation}
    \frac{\partial Q_{tot}}{\partial Q_i} \ge 0, \forall a \in A
    \label{eq:qmix:monotonic}
\end{equation}
A Hypernetwork \cite{ha2016hypernetworks} takes the true state $s$ as input and produces the parameters for the mixing networks, such that the constraint in Eq.\ref{eq:qmix:monotonic} is satisfied.
The mixing networks and individual utility functions $Q_i(\uptau^i, u^i; \theta^i)$ are jointly trained in a centralized fashion.
Then, when the trained agents can be deployed to a distributed environment, where each agent solely selects greedy actions with respect to its own utility function.
Interesingly, no communication between agents and centralizatize controller is required.


==> section/abstract.tex <==
\begin{abstract}
Distributed access control is a crucial component for \gls{mmtc}.
In this communication scenario, centralized resource allocation is not scalable because resource configurations have to be sent frequently from the base station to a massive number of devices.
We investigate distributed reinforcement learning for resource selection without relying on centralized control.
Another important feature of \gls{mmtc} is the sporadic and dynamic change of traffic.
Existing studies on distributed access control assume that traffic load is static or they are able to gradually adapt to the dynamic traffic.
We minimize the adaptation period by training TinyQMIX, which is a lightweight multi-agent deep reinforcement learning model, to learn a distributed wireless resource selection policy under various traffic patterns before deployment.
Therefore, the trained agents are able to quickly adapt to dynamic traffic and provide low access delay.
Numerical results are presented to support our claims.
\end{abstract}
\begin{IEEEkeywords}
    \gls{mmtc}, multi agent deep reinforcement learning
\end{IEEEkeywords}
\glsresetall


==> section/acknowledgement.tex <==
% \section*{Acknowledgment}

% The preferred spelling of the word ``acknowledgment'' in America is without 
% an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
% G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
% acknowledgments in the unnumbered footnote on the first page.


==> section/util/title.tex <==
\title{TinyQMIX: Distributed Access Control for mMTC via Multi-agent Reinforcement Learning
% {\footnotesize \textsuperscript{*}Note: Sub-titles are not captured in Xplore and
% should not be used}
%\thanks{Identify applicable funding agency here. If none, delete this.}
}

\author{
    \IEEEauthorblockN{
        Tien Thanh Le\IEEEauthorrefmark{1}\IEEEauthorrefmark{2}, 
        Yusheng Ji\IEEEauthorrefmark{2}\IEEEauthorrefmark{1}, 
        John C.S. Lui \IEEEauthorrefmark{3}
    }
    \IEEEauthorblockA{
        \IEEEauthorrefmark{1}Department of Informatics, The Graduate University for Advanced Studies, SOKENDAI, Tokyo, Japan\\
        \IEEEauthorrefmark{2}National Institute of Informatics, Tokyo, Japan\\
        \IEEEauthorrefmark{3}Department of Computer Science and Engineering, The Chinese University of Hong Kong, Hong Kong\\
        Email: \IEEEauthorrefmark{1}\IEEEauthorrefmark{2}\{lethanh, kei\}@nii.ac.jp;\IEEEauthorrefmark{3}cslui@cse.cuhk.edu.hk
    }
}

